AAS-VC: On the Generalization Ability of Automatic Alignment Search based Non-autoregressive Sequence-to-sequence Voice Conversion

Non-autoregressive (non-AR) sequence-to-seqeunce (seq2seq) models for voice conversion (VC) is attractive in its ability to effectively model the temporal structure while enjoying boosted intelligibility and fast inference thanks to non-AR modeling. However, the dependency of current non-AR seq2seq VC models on ground truth durations extracted from an external AR model greatly limits its generalization ability to smaller training datasets. In this paper, we first demonstrate the above-mentioned problem by varying the training data size. Then, we present AAS-VC, a non-AR seq2seq VC model based on automatic alignment search (AAS), which removes the dependency on external durations and serves as a proper inductive bias to provide the required generalization ability for small datasets. Experimental results show that AAS-VC can generalize better to a training dataset of only 5 minutes. We also conducted ablation studies to justify several model design choices. The audio samples and implementation are available online.

==> tables/unseen.tex <==
\begin{table}[h]
	\centering
	\caption{Objective comparison of using mel spectrograms and PPG as the source feature against seen and unseen source speakers, using 932 training utterances.}
        % \footnotesize
	
	\centering
        \begin{tabular}{c c | c c c c }
		\toprule
            \makecell{Source\\feature} & \makecell{Source\\speaker} & MCD & F0CORR & DDUR & CER \\
            \midrule
            \multirow{2}{*}[0pt]{mel} & seen & 6.35 & 0.450 & 0.193 & 3.4 \\
             & unseen & 8.09 & 0.144 & 0.524 & 47.3 \\
            \midrule
            \multirow{2}{*}[0pt]{PPG} & seen & 6.23 & 0.458 & 0.190 & 1.7 \\
             & unseen & 6.35 & 0.443 & 0.398 & 2.3 \\
            \bottomrule
	\end{tabular}
	\label{tab:unseen}
\end{table}
